Cache-Efficient Fork-Processing Patterns on Large Graphs

As large graph processing emerges, we observe a costly fork-processing pattern (FPP) that is common in many graph algorithms. The unique feature of the FPP is that it launches many independent queries from different source vertices on the same graph. For example, an algorithm in analyzing the network community profile can execute Personalized PageRanks that start from tens of thousands of source vertices at the same time. We study the efficiency of handling FPPs in state-of-the-art graph processing systems on multi-core architectures. We find that those systems suffer from severe cache miss penalty because of the irregular and uncoordinated memory accesses in processing FPPs. In this paper, we propose ForkGraph, a cache-efficient FPP processing system on multi-core architectures. To improve the cache reuse, we divide the graph into partitions each sized of LLC capacity, and the queries in an FPP are buffered and executed on the partition basis. We further develop efficient intra- and inter-partition execution strategies for efficiency. For intra-partition processing, since the graph partition fits into LLC, we propose to execute each graph query with efficient sequential algorithms (in contrast with parallel algorithms in existing parallel graph processing systems) and present an atomic-free query processing by consolidating contending operations to cache-resident graph partition. For inter-partition processing, we propose yielding and priority-based scheduling, to reduce redundant work in processing. Besides, we theoretically prove that ForkGraph performs the same amount of work, to within a constant factor, as the fastest known sequential algorithms in FPP queries processing, which is work efficient. Our evaluations on real-world graphs show that ForkGraph significantly outperforms state-of-the-art graph processing systems with two orders of magnitude speedups.

==> table/tbl_compare.tex <==

\resizebox{\textwidth}{!}{%
\begin{tabular}{|r|r|r|r|r|r|}
\hline
Implementation & Max Mem (GB) & LLC Misses / CGQ & Context Switches / CGQ & CPU Utilization & Avg Execution Time      \\ \hline
Ligra-S        & 5.6                            & $4.4\times 10^8$                   & 7404.44                        & $72\%$                    & 2.98 seconds                        \\ \hline
Ligra-O        & \phantom{0}\Bad{}\Bad{}111.6   & \phantom{0}\Bad{}$7.0\times 10^8$  & \phantom{0}\Bad{}\Bad{}12968.72& \phantom{0}\GoodR{}$100\%$ & \phantom{0}\Bad{}\Bad{}9.38 seconds \\ \hline
Ligra-C        & \phantom{0}\Bad{}7.6           & \phantom{0}\Bad{}$7.4\times 10^8$  & \phantom{0}\Good{}240.85       & \phantom{0}\GoodR{}$95\%$  & \phantom{0}\Good{}2.72 seconds      \\ \hline
\end{tabular}}

